Efficient Globally Convergent Stochastic Optimization for Canonical Correlation Analysis

We study the stochastic optimization of canonical correlation analysis (CCA), whose objective is nonconvex and does not decouple over training samples. Although several stochastic gradient based optimization algorithms have been recently proposed to solve this problem, no global convergence guarantee was provided by any of them. Inspired by the alternating least squares/power iterations formulation of CCA, and the shift-and-invert preconditioning method for PCA, we propose two globally convergent meta-algorithms for CCA, both of which transform the original problem into sequences of least squares problems that need only be solved approximately. We instantiate the meta-algorithms with state-of-the-art SGD methods and obtain time complexities that significantly improve upon that of previous work. Experimental results demonstrate their superior performance.

==> conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

%% We have proposed a globally convergent stochastic algorithm for CCA, whose objective is nonconvex and does not decouple over training samples. Our algorithm makes use of the alternating least squares/power iterations formulation of CCA, and solves the least squares problems approximately with state-of-the-art stochastic gradient descent methods. The overall time complexity of our algorithm significantly improves upon previous work both theoretically and empirically.

One straightforward application of our algorithm is approximate kernel CCA. % ~\cite{Lopez_14b}
% using random Fourier features~\cite{RahimiRecht08a}. % RahimiRecht09a 
The algorithm of~\cite{Lopez_14b} first maps original inputs into high dimensional random feature space and then performs linear CCA on top. We can solve the resulting high dimensional CCA problem with our stochastic algorithm, as done by~\cite{Xie_15b,WangLivesc16a}.
Another future direction is to extend the general inexact power iterations approach to other spectral dimension reduction algorithms (e.g., linear discriminant analysis is equivalent to CCA with proper representation for the class labels). % ~\cite{BachJordan05a}). 




==> log <==
pdflatex main
This is pdfTeX, Version 3.1415926-2.5-1.40.14 (TeX Live 2013)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2011/06/27>
Babel <v3.8m> and hyphenation patterns for english, dumylang, nohyphenation, lo
aded.
(/usr/share/texlive/texmf-dist/tex/latex/base/article.cls
Document Class: article 2007/10/19 v1.4h Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size10.clo)) (./nips_2016.sty
(/usr/share/texlive/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifpdf.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifvtex.sty)
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/base/inputenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/utf8.def
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.dfu)
(/usr/share/texlive/texmf-dist/tex/latex/base/ot1enc.dfu)
(/usr/share/texlive/texmf-dist/tex/latex/base/omsenc.dfu)))
(/usr/share/texlive/texmf-dist/tex/latex/base/fontenc.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/t1enc.def))
(/usr/share/texlive/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texlive/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/home-nfs/wwang5/texmf/tex/latex/units/nicefrac.sty
(/usr/share/texlive/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/microtype.cfg))
(/home-nfs/wwang5/texmf/tex/latex/algorithms/algorithm.sty
(/usr/share/texlive/texmf-dist/tex/latex/float/float.sty))
(/home-nfs/wwang5/texmf/tex/latex/algorithms/algorithmic.sty)
(/usr/share/texlive/texmf-dist/tex/latex/natbib/natbib.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/share/texlive/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/share/texlive/texmf-dist/tex/latex/psfrag/psfrag.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/graphics.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/pdftex-def/pdftex.def
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty))))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/color.sty
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/color.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty)
(/usr/share/texlive/texmf-dist/tex/latex/pdfpages/pdfpages.sty
(/usr/share/texlive/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texlive/texmf-dist/tex/latex/eso-pic/eso-pic.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/atbegshi.sty))
(/usr/share/texlive/texmf-dist/tex/latex/pdfpages/pppdftex.def))
(/home-nfs/wwang5/texmf/tex/latex/multirow/multirow.sty)
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texlive/texmf-dist/tex/latex/caption/caption3.sty)) (./MACPdef.tex)
 (./MACPdef-ams.tex) (/usr/share/texlive/texmf-dist/tex/latex/mh/mathtools.sty
(/usr/share/texlive/texmf-dist/tex/latex/mh/mhsetup.sty))
(/home-nfs/wwang5/texmf/tex/latex/eqparbox/eqparbox.sty
(/usr/share/texlive/texmf-dist/tex/latex/tools/array.sty)
(/home-nfs/wwang5/texmf/tex/latex/environ/environ.sty
(/home-nfs/wwang5/texmf/tex/latex/trimspaces/trimspaces.sty)))
No file main.aux.
(/usr/share/texlive/texmf-dist/tex/latex/psnfss/t1ptm.fd)
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
*geometry* verbose mode - [ preamble ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(92.14519pt, 430.00462pt, 92.14519pt)
* v-part:(T,H,B)=(95.39737pt, 556.47656pt, 143.09605pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=430.00462pt
* \textheight=556.47656pt
* \oddsidemargin=19.8752pt
* \evensidemargin=19.8752pt
* \topmargin=-13.87262pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

*geometry* verbose mode - [ newgeometry ] result:
* driver: pdftex
* paper: letterpaper
* layout: <same size as paper>
* layoutoffset:(h,v)=(0.0pt,0.0pt)
* modes: 
* h-part:(L,W,R)=(108.405pt, 397.48499pt, 108.40501pt)
* v-part:(T,H,B)=(72.26999pt, 650.43pt, 72.27pt)
* \paperwidth=614.295pt
* \paperheight=794.96999pt
* \textwidth=397.48499pt
* \textheight=650.43pt
* \oddsidemargin=36.13501pt
* \evensidemargin=36.13501pt
* \topmargin=-37.0pt
* \headheight=12.0pt
* \headsep=25.0pt
* \topskip=10.0pt
* \footskip=30.0pt
* \marginparwidth=65.0pt
* \marginparsep=11.0pt
* \columnsep=10.0pt
* \skip\footins=9.0pt plus 4.0pt minus 2.0pt
* \hoffset=0.0pt
* \voffset=0.0pt
* \mag=1000
* \@twocolumnfalse
* \@twosidefalse
* \@mparswitchfalse
* \@reversemarginfalse
* (1in=72.27pt=25.4mm, 1cm=28.453pt)

(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-ptm.cfg)
(/usr/share/texlive/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texlive/texmf-dist/tex/generic/oberdiek/pdftexcmds.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifluatex.sty))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvdefinekeys.sty))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvsetkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/etexcmds.sty)))
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texlive/texmf-dist/tex/latex/microtype/mt-msb.cfg)
(/usr/share/texlive/texmf-dist/tex/latex/base/t1cmtt.fd) (./intro.tex

Package natbib Warning: Citation `Hotell36a' on page 1 undefined on input line 
5.


Package natbib Warning: Citation `Vinod76a' on page 1 undefined on input line 1
0.


LaTeX Warning: Reference `e:cca' on page 1 undefined on input line 12.


LaTeX Warning: Reference `e:cca' on page 1 undefined on input line 22.


Package natbib Warning: Citation `Ma_15b' on page 1 undefined on input line 22.



Package natbib Warning: Citation `Wang_15c' on page 1 undefined on input line 2
2.


Package natbib Warning: Citation `Xie_15b' on page 1 undefined on input line 22
.

[1
Non-PDF special ignored!{/usr/share/texlive/texmf/fonts/map/pdftex/updmap/pdfte
x.map}]

LaTeX Warning: Reference `e:cca' on page 2 undefined on input line 24.


LaTeX Warning: Reference `alg:meta-alsvr' on page 2 undefined on input line 24.



LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 2 undefined on inp
ut line 24.


LaTeX Warning: Reference `e:cca' on page 2 undefined on input line 24.


LaTeX Warning: Reference `t:final' on page 2 undefined on input line 39.


LaTeX Warning: Reference `sec:svrg' on page 2 undefined on input line 40.


LaTeX Warning: Reference `sec:meta-shift-and-invert-time' on page 2 undefined o
n input line 40.


Package natbib Warning: Citation `Ma_15b' on page 2 undefined on input line 50.



Package natbib Warning: Citation `Ge_16a' on page 2 undefined on input line 51.


) (./motivation.tex

LaTeX Warning: Reference `e:cca' on page 2 undefined on input line 23.


Package natbib Warning: Citation `GolubZha95a' on page 2 undefined on input lin
e 23.


LaTeX Warning: Reference `alg:als' on page 2 undefined on input line 23.

[2]

LaTeX Warning: Reference `alg:als' on page 3 undefined on input line 50.


LaTeX Warning: Reference `alg:als' on page 3 undefined on input line 55.


LaTeX Warning: Reference `alg:als' on page 3 undefined on input line 69.


Package natbib Warning: Citation `GolubLoan96a' on page 3 undefined on input li
ne 69.


LaTeX Warning: Reference `append:proof-alternating-least-squares-exact' on page
 3 undefined on input line 71.


LaTeX Warning: Reference `e:cca' on page 3 undefined on input line 72.


LaTeX Warning: Reference `alg:als' on page 3 undefined on input line 74.


LaTeX Warning: Reference `alg:als' on page 3 undefined on input line 75.


LaTeX Warning: Reference `thm:alternating-least-squares-exact' on page 3 undefi
ned on input line 78.


LaTeX Warning: Reference `alg:als' on page 3 undefined on input line 80.


LaTeX Warning: Reference `e:lsq' on page 3 undefined on input line 84.

) (./algorithm1.tex [3]

Package natbib Warning: Citation `JohnsonZhang13a' on page 4 undefined on input
 line 56.


LaTeX Warning: Reference `alg:meta-alsvr' on page 4 undefined on input line 56.



Package natbib Warning: Citation `Ma_15b' on page 4 undefined on input line 65.



Package natbib Warning: Citation `Ma_15b' on page 4 undefined on input line 65.



Package natbib Warning: Citation `Wang_15c' on page 4 undefined on input line 6
5.


LaTeX Warning: Reference `alg:meta-alsvr' on page 4 undefined on input line 69.



Package natbib Warning: Citation `Ma_15b' on page 4 undefined on input line 69.



Package natbib Warning: Citation `Wang_15c' on page 4 undefined on input line 6
9.


Package natbib Warning: Citation `LuFoster14a' on page 4 undefined on input lin
e 71.

[4]

LaTeX Warning: Reference `alg:meta-alsvr' on page 5 undefined on input line 76.



LaTeX Warning: Reference `append:proof-alternating-least-squares-inexact' on pa
ge 5 undefined on input line 76.


LaTeX Warning: Reference `alg:meta-alsvr' on page 5 undefined on input line 76.



LaTeX Warning: Reference `alg:als' on page 5 undefined on input line 76.


LaTeX Warning: Reference `alg:meta-alsvr' on page 5 undefined on input line 78.



LaTeX Warning: Reference `alg:meta-alsvr' on page 5 undefined on input line 79.



Underfull \hbox (badness 1072) in paragraph at lines 79--81
[]\T1/ptm/b/it/10 Theorem \T1/ptm/m/n/10 (+20) 2 (Con-ver-gence of Al-go-rithm 
[])\T1/ptm/m/it/10 (+20) . []\T1/ptm/m/n/10 (+20) Fix $[][]$, and set $\OML/cmm
/m/it/10 ^^O\OT1/cmr/m/n/10 (\OML/cmm/m/it/10 T\OT1/cmr/m/n/10 ) \OMS/cmsy/m/n/
10 ^^T

LaTeX Warning: Reference `alg:meta-alsvr' on page 5 undefined on input line 87.



LaTeX Warning: Reference `e:lsq' on page 5 undefined on input line 87.


LaTeX Warning: Reference `e:lsq' on page 5 undefined on input line 87.


Package natbib Warning: Citation `Schmid_13a' on page 5 undefined on input line
 87.


Package natbib Warning: Citation `ShalevZhang13b' on page 5 undefined on input 
line 87.


Package natbib Warning: Citation `JohnsonZhang13a' on page 5 undefined on input
 line 87.


LaTeX Warning: Reference `e:lsq' on page 5 undefined on input line 87.


Package natbib Warning: Citation `Frostig_15a' on page 5 undefined on input lin
e 87.


Package natbib Warning: Citation `Lin_15a' on page 5 undefined on input line 87
.


LaTeX Warning: Reference `e:lsq' on page 5 undefined on input line 88.


LaTeX Warning: Reference `append:alg-svrg' on page 5 undefined on input line 88
.


LaTeX Warning: Reference `append:meta-alternating-least-squares-initial-subopti
mality' on page 5 undefined on input line 91.


Package natbib Warning: Citation `JohnsonZhang13a' on page 5 undefined on input
 line 91.


Package natbib Warning: Citation `Lin_15a' on page 5 undefined on input line 91
.


Package natbib Warning: Citation `JohnsonZhang13a' on page 5 undefined on input
 line 93.


Package natbib Warning: Citation `Lin_15a' on page 5 undefined on input line 99
.


Package natbib Warning: Citation `Lin_15a' on page 5 undefined on input line 10
5.


LaTeX Warning: Reference `thm:alternating-least-squares-inexact' on page 5 unde
fined on input line 107.


LaTeX Warning: Reference `lem:svrg' on page 5 undefined on input line 107.


Package natbib Warning: Citation `Ma_15b' on page 5 undefined on input line 109
.


Package natbib Warning: Citation `Nester04a' on page 5 undefined on input line 
109.

) (./algorithm2.tex
Underfull \hbox (badness 2653) in paragraph at lines 107--1
[]\T1/ptm/m/n/10 (+20) By com-bin-ing the it-er-a-tion com-plex-ity of the oute
r loop (The-o-rem []) and the time

Underfull \hbox (badness 4048) in paragraph at lines 107--1
\T1/ptm/m/n/10 (+20) com-plex-ity of the in-ner loop (Lemma []), we ob-tain the
 to-tal time com-plex-ity of

Package natbib Warning: Citation `GarberHazan15c' on page 5 undefined on input 
line 90.


Package natbib Warning: Citation `Jin_15a' on page 5 undefined on input line 90
.


LaTeX Warning: Reference `e:C-def' on page 5 undefined on input line 90.


Underfull \vbox (badness 1762) has occurred while \output is active [5]

LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 6 undefined on inp
ut line 124.


LaTeX Warning: Reference `append:alg-shift-and-invert' on page 6 undefined on i
nput line 124.


Overfull \hbox (14.22044pt too wide) in paragraph at lines 203--203
[] 

LaTeX Warning: Reference `append:proof-shift-and-invert-phase-I' on page 6 unde
fined on input line 225.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 6 undefined on inp
ut line 227.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 6 undefined on inp
ut line 238.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 6 undefined on inp
ut line 239.


LaTeX Warning: Reference `e:normal-3' on page 6 undefined on input line 239.

[6]

LaTeX Warning: Reference `e:cca' on page 7 undefined on input line 260.


LaTeX Warning: Reference `append:proof-shift-and-invert-phase-II' on page 7 und
efined on input line 261.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 7 undefined on inp
ut line 263.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 7 undefined on inp
ut line 264.


LaTeX Warning: Reference `e:phaseI-2-main' on page 7 undefined on input line 26
4.


LaTeX Warning: Reference `e:final-normal' on page 7 undefined on input line 264
.


LaTeX Warning: Reference `e:cca' on page 7 undefined on input line 265.


LaTeX Warning: Reference `thm:shift-and-invert-phase-I' on page 7 undefined on 
input line 272.


LaTeX Warning: Reference `e:new-lsq-3' on page 7 undefined on input line 272.


LaTeX Warning: Reference `e:normal-3' on page 7 undefined on input line 272.


LaTeX Warning: Reference `e:new-lsq-3' on page 7 undefined on input line 272.


LaTeX Warning: Reference `e:final-normal' on page 7 undefined on input line 272
.


LaTeX Warning: Reference `e:new-lsq-3' on page 7 undefined on input line 273.


LaTeX Warning: Reference `e:new-lsq-3' on page 7 undefined on input line 273.


LaTeX Warning: Reference `thm:shift-and-invert-phase-I' on page 7 undefined on 
input line 304.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 7 undefined on inp
ut line 304.


LaTeX Warning: Reference `lem:shift-and-invert-repeat-until' on page 7 undefine
d on input line 304.


LaTeX Warning: Reference `append:proof-shift-and-invert-iteration-complexity' o
n page 7 undefined on input line 304.


LaTeX Warning: Reference `append:cond-h' on page 7 undefined on input line 305.



LaTeX Warning: Reference `lem:shift-and-invert-cond-svrg' on page 7 undefined o
n input line 305.


Package natbib Warning: Citation `GarberHazan15c' on page 7 undefined on input 
line 307.


LaTeX Warning: Reference `t:final' on page 7 undefined on input line 309.


Package natbib Warning: Citation `Ge_16a' on page 7 undefined on input line 314
.


LaTeX Warning: Reference `sec:svrg' on page 7 undefined on input line 315.

[7]

Package natbib Warning: Citation `Witten_09a' on page 8 undefined on input line
 329.


Package natbib Warning: Citation `GolubLoan96a' on page 8 undefined on input li
ne 329.


Package natbib Warning: Citation `Ma_15b' on page 8 undefined on input line 330
.


Package natbib Warning: Citation `Wang_15c' on page 8 undefined on input line 3
30.

) (./experiments.tex

Package natbib Warning: Citation `Snoek_06a' on page 8 undefined on input line 
6.


Package natbib Warning: Citation `Westbur94a' on page 8 undefined on input line
 6.


Package natbib Warning: Citation `Lecun_98a' on page 8 undefined on input line 
6.


Package natbib Warning: Citation `Ma_15b' on page 8 undefined on input line 7.


Package natbib Warning: Citation `Ge_16a' on page 8 undefined on input line 7.


LaTeX Warning: Reference `fig:real_data' on page 8 undefined on input line 9.


LaTeX Warning: Reference `append:expts' on page 8 undefined on input line 9.

<figures/mediamill_100000-eps-converted-to.pdf, id=50, 401.5pt x 293.095pt>
<use figures/mediamill_100000-eps-converted-to.pdf>
<figures/mediamill_10000-eps-converted-to.pdf, id=51, 408.52625pt x 293.095pt>
<use figures/mediamill_10000-eps-converted-to.pdf>
<figures/mediamill_1000-eps-converted-to.pdf, id=52, 397.485pt x 293.095pt>
<use figures/mediamill_1000-eps-converted-to.pdf>
<figures/mediamill_100-eps-converted-to.pdf, id=53, 398.48875pt x 293.095pt>
<use figures/mediamill_100-eps-converted-to.pdf>
<figures/jw11_100000-eps-converted-to.pdf, id=54, 401.5pt x 293.095pt>
<use figures/jw11_100000-eps-converted-to.pdf>
<figures/jw11_10000-eps-converted-to.pdf, id=55, 401.5pt x 293.095pt>
<use figures/jw11_10000-eps-converted-to.pdf>
<figures/jw11_1000-eps-converted-to.pdf, id=56, 408.52625pt x 293.095pt>
<use figures/jw11_1000-eps-converted-to.pdf>
<figures/jw11_100-eps-converted-to.pdf, id=57, 398.48875pt x 297.11pt>
<use figures/jw11_100-eps-converted-to.pdf>
<figures/mnist_100000-eps-converted-to.pdf, id=58, 401.5pt x 293.095pt>
<use figures/mnist_100000-eps-converted-to.pdf>
<figures/mnist_10000-eps-converted-to.pdf, id=59, 408.52625pt x 293.095pt>
<use figures/mnist_10000-eps-converted-to.pdf>
<figures/mnist_1000-eps-converted-to.pdf, id=60, 408.52625pt x 293.095pt>
<use figures/mnist_1000-eps-converted-to.pdf>
<figures/mnist_100-eps-converted-to.pdf, id=61, 398.48875pt x 293.095pt>
<use figures/mnist_100-eps-converted-to.pdf>
Overfull \hbox (1.7338pt too wide) in paragraph at lines 14--51
 [][] 
) [8] [9 <./figures/mediamill_100000-eps-converted-to.pdf> <./figures/mediamill
_10000-eps-converted-to.pdf> <./figures/mediamill_1000-eps-converted-to.pdf> <.
/figures/mediamill_100-eps-converted-to.pdf> <./figures/jw11_100000-eps-convert
ed-to.pdf> <./figures/jw11_10000-eps-converted-to.pdf> <./figures/jw11_1000-eps
-converted-to.pdf> <./figures/jw11_100-eps-converted-to.pdf> <./figures/mnist_1
00000-eps-converted-to.pdf> <./figures/mnist_10000-eps-converted-to.pdf> <./fig
ures/mnist_1000-eps-converted-to.pdf> <./figures/mnist_100-eps-converted-to.pdf
>] (./main.bbl) [10] (./append1.tex

LaTeX Warning: Reference `thm:alternating-least-squares-exact' on page 11 undef
ined on input line 1.


LaTeX Warning: Reference `alg:als' on page 11 undefined on input line 5.


LaTeX Warning: Reference `alg:als' on page 11 undefined on input line 15.


Underfull \vbox (badness 2150) has occurred while \output is active [11]

LaTeX Warning: Reference `thm:alternating-least-squares-inexact' on page 12 und
efined on input line 56.


LaTeX Warning: Reference `alg:meta-alsvr' on page 12 undefined on input line 59
.


LaTeX Warning: Reference `alg:als' on page 12 undefined on input line 59.


LaTeX Warning: Reference `alg:als' on page 12 undefined on input line 63.


LaTeX Warning: Reference `alg:meta-alsvr' on page 12 undefined on input line 63
.


LaTeX Warning: Reference `alg:meta-alsvr' on page 12 undefined on input line 64
.


LaTeX Warning: Reference `alg:meta-alsvr' on page 12 undefined on input line 72
.


LaTeX Warning: Reference `e:split-errors-1' on page 12 undefined on input line 
87.


LaTeX Warning: Reference `e:split-errors-1' on page 12 undefined on input line 
93.

[12]

LaTeX Warning: Reference `alg:als' on page 13 undefined on input line 115.


LaTeX Warning: Reference `e:split-errors-1' on page 13 undefined on input line 
119.


LaTeX Warning: Reference `e:split-errors-2' on page 13 undefined on input line 
119.


LaTeX Warning: Reference `e:split-errors-3' on page 13 undefined on input line 
119.


LaTeX Warning: Reference `e:split-errors-3' on page 13 undefined on input line 
126.


LaTeX Warning: Reference `thm:alternating-least-squares-inexact' on page 13 und
efined on input line 130.


LaTeX Warning: Reference `lem:alternating-least-squares-distance' on page 13 un
defined on input line 133.


LaTeX Warning: Reference `thm:alternating-least-squares-exact' on page 13 undef
ined on input line 142.


LaTeX Warning: Reference `lem:alternating-least-squares-distance' on page 13 un
defined on input line 142.


LaTeX Warning: Reference `alg:meta-alsvr' on page 13 undefined on input line 14
2.


LaTeX Warning: Reference `e:inexact-last-step' on page 13 undefined on input li
ne 142.


LaTeX Warning: Reference `e:lsq' on page 13 undefined on input line 151.

[13]

LaTeX Warning: Reference `alg:meta-alsvr' on page 14 undefined on input line 17
5.

) [14] (./append2.tex

LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 15 undefined on in
put line 4.


LaTeX Warning: Reference `thm:shift-and-invert-phase-I' on page 15 undefined on
 input line 91.


LaTeX Warning: Reference `thm:shift-and-invert-phase-I' on page 15 undefined on
 input line 178.


Package natbib Warning: Citation `GarberHazan15c' on page 15 undefined on input
 line 178.


Underfull \vbox (badness 10000) has occurred while \output is active [15]

Package natbib Warning: Citation `GarberHazan15c' on page 16 undefined on input
 line 193.

(/usr/share/texlive/texmf-dist/tex/latex/psnfss/omsptm.fd)

Package natbib Warning: Citation `GarberHazan15c' on page 16 undefined on input
 line 237.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 16 undefined on in
put line 238.


LaTeX Warning: Reference `e:SI-bound-distance' on page 16 undefined on input li
ne 294.


LaTeX Warning: Reference `e:SI-bound-distance' on page 16 undefined on input li
ne 294.


LaTeX Warning: Reference `lem:shift-and-invert-exact' on page 16 undefined on i
nput line 295.

[16]

Package natbib Warning: Citation `GarberHazan15c' on page 17 undefined on input
 line 323.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 17 und
efined on input line 326.


Underfull \hbox (badness 2478) in paragraph at lines 328--329
[]\T1/ptm/m/n/10 (+20) (crude regime) Let $\OML/cmm/m/it/10 t[] \OT1/cmr/m/n/10
 = [][] [] [][]$\T1/ptm/m/n/10 (+20) . Fix $\OML/cmm/m/it/10 T \OMS/cmsy/m/n/10
 ^^U \OML/cmm/m/it/10 t[]$\T1/ptm/m/n/10 (+20) , and set $[]\OT1/cmr/m/n/10 (\O
ML/cmm/m/it/10 T\OT1/cmr/m/n/10 ) =

LaTeX Warning: Reference `e:new-lsq' on page 17 undefined on input line 351.

[17]

LaTeX Warning: Reference `e:SI-bound-distance' on page 18 undefined on input li
ne 452.


LaTeX Warning: Reference `lem:shift-and-invert-exact' on page 18 undefined on i
nput line 465.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 18 und
efined on input line 511.


LaTeX Warning: Reference `e:SI-split-errors-1' on page 18 undefined on input li
ne 519.

[18]

LaTeX Warning: Reference `e:SI-split-errors-1' on page 19 undefined on input li
ne 542.


LaTeX Warning: Reference `e:SI-split-errors-2' on page 19 undefined on input li
ne 542.


LaTeX Warning: Reference `e:SI-split-errors-3' on page 19 undefined on input li
ne 542.


LaTeX Warning: Reference `e:SI-split-errors-3' on page 19 undefined on input li
ne 548.


LaTeX Warning: Reference `lem:shift-and-invert-inexact' on page 19 undefined on
 input line 551.


LaTeX Warning: Reference `lem:shift-and-invert-exact' on page 19 undefined on i
nput line 566.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 19 und
efined on input line 566.


LaTeX Warning: Reference `e:SI-inexact-1' on page 19 undefined on input line 56
6.


LaTeX Warning: Reference `lem:shift-and-invert-exact' on page 19 undefined on i
nput line 575.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 19 und
efined on input line 575.


LaTeX Warning: Reference `e:SI-inexact-2' on page 19 undefined on input line 57
5.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 19 undefined on in
put line 581.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 19 undefined on in
put line 584.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 19 und
efined on input line 584.

[19]

LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 20 undefined on in
put line 588.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 20 undefined on in
put line 589.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 20 und
efined on input line 611.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 20 undefined on in
put line 619.


LaTeX Warning: Reference `e:SI-bound-distance' on page 20 undefined on input li
ne 619.


LaTeX Warning: Reference `e:delta-s-1' on page 20 undefined on input line 634.


LaTeX Warning: Reference `e:delta-s-2' on page 20 undefined on input line 634.

[20]

LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 21 undefined on in
put line 641.


LaTeX Warning: Reference `e:lambda-recurse' on page 21 undefined on input line 
654.


LaTeX Warning: Reference `e:lambda-recurse' on page 21 undefined on input line 
661.


LaTeX Warning: Reference `e:lambda-recurse' on page 21 undefined on input line 
664.


LaTeX Warning: Reference `e:lambda-recurse-2' on page 21 undefined on input lin
e 672.


LaTeX Warning: Reference `e:delta-s-1' on page 21 undefined on input line 679.


LaTeX Warning: Reference `e:epsilon-1' on page 21 undefined on input line 679.


LaTeX Warning: Reference `e:delta-s-1' on page 21 undefined on input line 691.

[21]

LaTeX Warning: Reference `e:epsilon-1' on page 22 undefined on input line 698.


LaTeX Warning: Reference `e:epsilon-2' on page 22 undefined on input line 715.


LaTeX Warning: Reference `e:epsilon-3' on page 22 undefined on input line 715.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 22 undefined on in
put line 718.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 22 undefined on in
put line 720.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 22 undefined on in
put line 721.


LaTeX Warning: Reference `e:delta-s-interval' on page 22 undefined on input lin
e 734.


LaTeX Warning: Reference `lem:shift-and-invert-inexact-distance' on page 22 und
efined on input line 736.


LaTeX Warning: Reference `e:epsilon-4' on page 22 undefined on input line 742.


LaTeX Warning: Reference `e:kappa-f' on page 22 undefined on input line 747.


LaTeX Warning: Reference `e:epsilon-3' on page 22 undefined on input line 748.


LaTeX Warning: Reference `thm:shift-and-invert-phase-I' on page 22 undefined on
 input line 756.


LaTeX Warning: Reference `lem:shift-and-invert-for-loop' on page 22 undefined o
n input line 757.

[22]

LaTeX Warning: Reference `thm:shift-and-invert-phase-II' on page 23 undefined o
n input line 767.


LaTeX Warning: Reference `e:phaseI-2' on page 23 undefined on input line 771.


LaTeX Warning: Reference `e:align-tailing' on page 23 undefined on input line 7
75.


LaTeX Warning: Reference `e:phaseI-2' on page 23 undefined on input line 775.


LaTeX Warning: Reference `e:normal-3' on page 23 undefined on input line 796.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 23 undefined on in
put line 803.

[23]

LaTeX Warning: Reference `lem:shift-and-invert-repeat-until' on page 24 undefin
ed on input line 836.


LaTeX Warning: Reference `alg:meta-shift-and-invert' on page 24 undefined on in
put line 836.

) (./append3.tex

LaTeX Warning: Reference `t:real_data' on page 24 undefined on input line 5.


Package natbib Warning: Citation `Ma_15b' on page 24 undefined on input line 5.



Package natbib Warning: Citation `Wang_15c' on page 24 undefined on input line 
5.


Package natbib Warning: Citation `Ma_15b' on page 24 undefined on input line 20
.


Package natbib Warning: Citation `WarmutKuzmin08a' on page 24 undefined on inpu
t line 26.


Package natbib Warning: Citation `Arora_12a' on page 24 undefined on input line
 26.


Package natbib Warning: Citation `Balsub_13a' on page 24 undefined on input lin
e 26.


Package natbib Warning: Citation `Shamir15a' on page 24 undefined on input line
 26.


Package natbib Warning: Citation `Xie_15b' on page 24 undefined on input line 2
6.


Package natbib Warning: Citation `GarberHazan15c' on page 24 undefined on input
 line 26.


Package natbib Warning: Citation `Jin_15a' on page 24 undefined on input line 2
6.


Package natbib Warning: Citation `Arora_12a' on page 24 undefined on input line
 28.

[24]

Package natbib Warning: Citation `Yger_12a' on page 25 undefined on input line 
31.


Package natbib Warning: Citation `Ma_15b' on page 25 undefined on input line 31
.


Package natbib Warning: Citation `Wang_15c' on page 25 undefined on input line 
31.


Package natbib Warning: Citation `Xie_15b' on page 25 undefined on input line 3
1.


LaTeX Warning: Reference `e:cca' on page 25 undefined on input line 31.

)

Package natbib Warning: There were undefined citations.

[25] (./main.aux

Package natbib Warning: Citation(s) may have changed.
(natbib)                Rerun to get citations correct.


! Package natbib Error: Bibliography not compatible with author-year citations.

(natbib)                Press <return> to continue in numerical citation style.


See the natbib package documentation for explanation.
Type  H <return>  for immediate help.
 ...                                              
                                                  
l.176 ...and\NAT@force@numbers{}\NAT@force@numbers
                                                  
? {/usr/share/texlive/texmf-dist/fonts/enc/dvips/base/8r.enc}{/usr/share/texlive/
texmf-dist/fonts/enc/dvips/cm-super/cm-super-t1.enc}</usr/share/texlive/texmf-d
ist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/share/texlive/texmf-dist/fo
nts/type1/public/amsfonts/cm/cmbx12.pfb></usr/share/texlive/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmbx7.pfb></usr/share/texlive/texmf-dist/fonts/type1/pub
lic/amsfonts/cm/cmbx9.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/ams
fonts/cm/cmex10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/
cmextra/cmex7.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm
/cmmi10.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi1
2.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi5.pfb><
/usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi6.pfb></usr/sh
are/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi7.pfb></usr/share/tex
live/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi8.pfb></usr/share/texlive/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmmi9.pfb></usr/share/texlive/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmmib10.pfb></usr/share/texlive/texmf-dist/fon
ts/type1/public/amsfonts/cmextra/cmmib7.pfb></usr/share/texlive/texmf-dist/font
s/type1/public/amsfonts/cm/cmr10.pfb></usr/share/texlive/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr12.pfb></usr/share/texlive/texmf-dist/fonts/type1/public
/amsfonts/cm/cmr5.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfont
s/cm/cmr6.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr
7.pfb></usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmr9.pfb></
usr/share/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy10.pfb></usr/sh
are/texlive/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy5.pfb></usr/share/tex
live/texmf-dist/fonts/type1/public/amsfonts/cm/cmsy6.pfb></usr/share/texlive/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmsy7.pfb></usr/share/texlive/texmf-dis
t/fonts/type1/public/amsfonts/cm/cmsy9.pfb></usr/share/texlive/texmf-dist/fonts
/type1/public/amsfonts/symbols/msbm10.pfb></usr/share/texlive/texmf-dist/fonts/
type1/public/amsfonts/symbols/msbm7.pfb></usr/share/texlive/texmf-dist/fonts/ty
pe1/public/cm-super/sftt1000.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw
/times/utmb8a.pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/share/texlive/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/share
/texlive/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on main.pdf (25 pages, 561441 bytes).
Transcript written on main.log.


==> related.tex <==
\section{Other related work}
\label{sec:related}

Recent years have witnessed continuous efforts to scale up fundamental methods such as principal component analysis (PCA) and partial least squares with stochastic/online updates~\cite{WarmutKuzmin08a,Arora_12a,Balsub_13a,Shamir15a,Xie_15b,GarberHazan15c,Jin_15a}. 
% {Krasul69a,OjaKarhun85a,WarmutKuzmin08a,Arora_12a,Arora_13a,Mitliag_13a,Balsub_13a,Shamir15a,Xie_15b,GarberHazan15c,Jin_15a,Frostig_16a}. 
But as pointed out by~\cite{Arora_12a}, the CCA objective is more challenging due to the constraints. 
% Our algorithm is inspired by the stochastic PCA algorithm of~\cite{GarberHazan15c} which transforms the nonconvex PCA objective into a small number of well-conditioned regularized least squares problems (solved by SVRG) through shifting and inverting the covariance matrix and running power iterations on the transformed matrix. For CCA, the alternating least squares formulation (Algorithm~\ref{alg:als}) already reduces to solving convex regularized least squares problems.

\cite{Yger_12a} proposed an adaptive CCA algorithm with efficient online updates based on matrix manifolds defined by the constraints. However, the goal of their algorithm is anomaly detection for streaming data with a varying distribution, rather than to optimize the CCA objective on a given dataset. Similar to our algorithms, the stochastic CCA algorithms of~\cite{Ma_15b,Wang_15c} are motivated by the ALS formulation. \cite{Xie_15b} proposed a stochastic algorithm based on the Lagrangian formulation of the objective~\eqref{e:cca}. None of these online/stochastic algorithms have rigorous global convergence guarantee.

% From an orthogonal direction, \cite{Avron_13a} and~\cite{Paul15a} propose randomized sample selection algorithms to scale up linear CCA. Their goal is to select a subset of paired examples, whose canonical correlation well approximates that of the entire training set. We note that it is also possible to apply sampling techniques for solving least squares problems in our algorithm in place of SVRG.

%% In a parallel work~\cite{Ge_16a}, the authors independently proposed a similar ALS meta-algorithm\footnote{Our arxiv preprints for the ALS algorithm was posted before their paper got accepted by ICML 2016.}, and they solve the least squares problems using AGD. The time complexity of their algorithm for extracting the first canonical correlation is $\tilde{\calO} \left( d N \sqrt{\kappa^\prime} \, \frac{\rho_1^2}{\rho_1^2 - \rho_2^2} \cdot \log \left(\frac{1}{\eta} \right) \right)$, %\cdot \texttt{polylog} \left(\frac{\rho_1^2}{\rho_1^2 - \rho_2^2}, \frac{1}{\mu} \right)  \right)$, which has linear dependence on $\frac{\rho_1^2}{\rho_1^2 - \rho_2^2} \log \left(\frac{1}{\eta} \right)$ (so their algorithm is overall linearly convergent, but our complexity for ALS+AGD has quadratic dependence on this factor), but typically worse dependence on $N$ and $\kappa^\prime$ (see also the remarks in Section~\ref{sec:svrg}). Moreover, our SI algorithm tends to significantly outperform ALS both theoretically and empirically. It is future work to remove extra $\log\left(\frac{1}{\eta}\right)$ dependence in our analysis.

